Partial Compilation of Variational Algorithms for Noisy Intermediate-Scale Quantum Machines

Quantum computing is on the cusp of reality with Noisy Intermediate-Scale Quantum (NISQ) machines currently under development and testing. Some of the most promising algorithms for these machines are variational algorithms that employ classical optimization coupled with quantum hardware to evaluate the quality of each candidate solution. Recent work used GRadient Descent Pulse Engineering (GRAPE) to translate quantum programs into highly optimized machine control pulses, resulting in a significant reduction in the execution time of programs. This is critical, as quantum machines can barely support the execution of short programs before failing. However, GRAPE suffers from high compilation latency, which is untenable in variational algorithms since compilation is interleaved with computation. We propose two strategies for partial compilation, exploiting the structure of variational circuits to pre-compile optimal pulses for specific blocks of gates. Our results indicate significant pulse speedups ranging from 1.5x-3x in typical benchmarks, with only a small fraction of the compilation latency of GRAPE.

==> Makefile <==
PDF = sample-micro52.pdf

all: ${PDF}

%.pdf: %.tex acmart.cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

clean:
	$(RM) *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.gz *.zip *.rpi \
  $(PDF) *-converted-to.pdf


==> txt/Thomas.tex <==
Problem:
Before the break, I was having trouble getting every uccsd lih slice to converge for the same pulse time for every angle (e.g. a slice would converge to 1e-3 error for angle 50 degrees at 20 nanoseconds but the same slice would not converge to 1e-3 error for angle 55 degrees at 20 nanoseconds). The pulse time for each slice was determined by using one randomly generated angle value, and binary searching for the lowest pulse time that QOC was able to reach 1e-3 error.

Failed Attempts:
My first attempt at solving this problem was to seed grape with the pulse of an adjacent angle, e.g. 55 degrees gets seeded with the pulse from 50 degrees. This was ineffective. The angles that were not converging reached the same local minimum that they were reaching before, but in fewer iterations. I then tried some different methods such as a scheme I dubbed “binary search w/ backoff” where I would increment the pulse time of an angle that was not converging. E.g. if 50 degrees converges to 20 ns, but 55 deg does not, we would try 55 deg at 22 ns. This was also ineffective and the non-converging angles appeared to reach similar minimums.

Choosing hyperparameters:
I used hyperopt, a hyperparameter (hp) optimizer, to search for the best learning rate and decay values for each slice on a combination of different pulse times and angles. Hyperopt was trying to find the learning rate and decay values that gave the slice the lowest error (I set no convergence target). From a brief scrub of the data, I chose the learning rate and decay value that appeared to work for multiple angles and multiple time values. This hp combination occurred with enough consistency that it appeared to be AGNOSTIC of the pulse time and angle of the slice. The combination was frequently achieving error rates of 1e-7.

Choosing a pulse time for each slice:
With my hyperparameters chosen, I binary searched for the lowest pulse time for which the slice was able to converge to 1e-5 error. Each slice was set to the same random angle as chosen before.

Obtaining pulses for every slice at every angle, for a fixed pulse time:
Using my hyperparameters, and the pulse times chosen for each slice, I ran QOC at angle increments of 5 degrees from [0, …, 355] in attempt to get 1e-3 error on each pulse.

Results:
Results stated are currently only for slices s0, s1, s2, s3 which each have 2 theta-dependent gates each (see discussion). Without hyperparameters, and using a binary search time for each slice that reached 1e-3 error, `125 of 286` pulses did not converge to 1e-3 error and it took `40mins on 14 cores`. With hyperparameters, and using a binary search time for each slice that reached 1e-5 error, `15 of 286` pulses did not converge to 1e-3 error and it took `3mins on 14 cores`.

Discussion:
I think choosing hyperparameters well and using a pulse time that achieves an error lower than the one we hope to achieve for our pre-compiled pulses is about as “uniform” as we are going to get in terms of being able to specify one pulse time for a slice. The results I have are currently only for the first 4 slices because I believe a different set of hyperparameters works better for the latter 4. It appears that choosing learning rate proportional to circuit depth yields good results. I am currently running hyperparameter optimization on the latter 4 slices to see what good hyperparameter choices are. Also, we would have to find good hyperparameter choices for QOC on the full circuit as well. Otherwise we would run into the same problem of not being able to choose one pulse time for which the full circuit converges to 1e-3 for every angle. Therefore, our flexible approach is not “hurt” by the need to choose good hyperparameters.
